Measuring sampling plan utility in post-marketing surveillance of medical products

Ensuring product quality is critical to combating the global challenge of substandard and falsified medical products. Post-marketing surveillance is a central quality-assurance activity in which products from consumer-facing locations are collected and tested. Regulators in low-resource settings use post-marketing surveillance to evaluate product quality across locations and determine corrective actions. Part of post-marketing surveillance is developing a sampling plan, which specifies where to test and the number of tests to conduct at a location. With limited resources, it is important to base decisions on the utility of the samples tested. We propose a Bayesian approach to generate a comprehensive utility metric for sampling plans. This sampling plan utility integrates regulatory risk assessments with prior testing data, available supply-chain information, and valuations of regulatory objectives. We develop an efficient method for calculating sampling plan utility. We illustrate the value of the utility metric with a case study based on de-identified post-marketing surveillance data from a low-resource setting.

==> tikz/tikz_FastEstAlg.tex <==


\usetikzlibrary{shapes.geometric}
% Define block styles
\begin{tikzpicture}[
squarednode/.style={rectangle, draw=gray!60, fill=gray!25, very thick,minimum height = 1.5cm,text width=2.5cm, align=center},
squarednode2/.style={rectangle, draw=gray!60, fill=gray!25, very thick,minimum height = 1.5cm,text width=4.5cm, align=center},
rectnode/.style={rectangle, draw=blue!60, fill=blue!25, very thick,  minimum height = 1.5cm, text width=2.8cm, align=center},
rectnode2/.style={rectangle, draw=blue!60, fill=blue!25, very thick,  minimum height = 1.5cm, text width=2cm, align=center},
rectnode3/.style={rectangle, draw=blue!60, fill=blue!25, dashed,  minimum height = 5cm, text width=5cm, align=left},
rectnode4/.style={rectangle, draw=blue!60, fill=blue!25, dashed, thick,  minimum height = 3.85cm, text width=3.1cm, align=left},
rectnode5/.style={rectangle, draw=blue!60, fill=blue!25, dashed,  minimum height = 2.7cm, text width=1cm, align=left},
rectnode6/.style={rectangle, draw=blue!60, fill=blue!25, very thick,  minimum height = 6.15cm, text width=7.5cm, align=left},
% node distance=10mm
]
%Nodes
\node[squarednode](p1){\footnotesize Get $\bm{L}_{ij}$};
\node[rectnode](o1)[above= 2.3cm of p1] {\small $L:(\gamma,\gamma)\rightarrow\mathrm{R}$};
\node[rectnode6](o6)[right = 1.8cm of o1]  {\footnotesize $\Gamma\overset{{\text{MCMC}}}{\sim}\dataSet$};
\node[rectnode3](o2)[right=3.7cm of o1] { $\Gamma_{\text{cand}}$};
\node[rectnode2](o3)[right=2.3cm of o2] {\footnotesize $\allocVec$, $\sourcingMat$};
\node[rectnode4](o4)[right= 5cm of o1] { $\Gamma_{\text{truth}}$};
\node[rectnode5](o5)[right= 6.5cm of o1] { $\Gamma_{\text{data}}$};
\node[squarednode](p2)[below = 2.3cm of o3]  {\footnotesize Generate $\dataSetNext$};
\node[squarednode](p3)[below = 1.3cm of p2]  {\footnotesize Get binomial likelihood $\bm{W}_{jm}$};
\node[squarednode2](p4)[below = 6cm of o2]  {\footnotesize Get minimum $v_j$ of each column $(\bm{L}\times\bm{W})_{\cdot j}$};
\node[squarednode2](p5)[below = 1.0cm of p4]  {\footnotesize Return average $v_j$};


%Lines
% \draw[thick,-] (i1) to  node[pos=0.5, left] {\normalsize{$\frac{3}{6}$}} (o1) ;
\draw[thick,->] (o2) to  node[pos=0.7, above] {\normalsize{$\gamma_i$}} (p1) ;
\draw[thick,->] (o1) to  node {}  (p1) ;
\draw[thick,->] (o4) -- + (-2.5,-2.1) |-  node[pos=0.6, above] {\normalsize{$\gamma_j$}}  (p1) ;
\draw[thick,->] (o5) -- + (3.5,-2.1) |-  node[pos=-0.01, above] {\normalsize{$\gamma_m$}}  (p2) ;
\draw[thick,->] (o3) to  node {} (p2) ;
\draw[thick,->] (p2) to  node[pos=0.6, right] {$\dataSetNext$} (p3) ;
\draw[thick,->] (o4) -- + (2.5,-2.1) |-  node[pos=0.4, right] {\normalsize{$\gamma_j$}}  (p3) ;
\draw[thick,->] (p1) to  node[pos=0.6, above] {$\bm{L}$} (p4) ;
\draw[thick,->] (p3) to  node[pos=0.6, above] {$\bm{W}$} (p4) ;
\draw[thick,->] (p4) to  node[pos=0.5, right] {$v_j$} (p5) ;

% \draw[thick,-] (p1) to  node[pos=0.96, above] {\normalsize{$\frac{0}{2}$}} (o3) ;

%\draw[thick,->] (i1) to node[very near end,above] {{$\frac{0}{12}$}} (o2);
% \draw[thick,-] (i2) to node[pos=0.96, above] {\normalsize{$\frac{0}{9}$}} (o1);
% \draw[thick,-] (p2) to node[pos=0.97, above] {} (o2);
% \draw[thick,-] (p2) to node[pos=0.85, right] {} (o3);
% \draw[thick,->] (i3) to node[right] {{$\frac{0}{12}$}} (o3);
% \draw[thick,->] (i3) to node[above] {{$\frac{0}{12}$}} (o2);

% Make a legend
% \matrix [draw,below left] at (current bounding box.south west) {
%   \node [roundnode,label=right:Foo] {}; \\
%   \node [squarednode,label=right:Bar] {}; \\
% };

% \node[draw,left = 1.5cm of o1,minimum height=1.1cm,minimum width=2.5cm] (lgd) {$\frac{\text{\footnotesize positive tests}}{\text{\footnotesize total samples}}$};

% Other possible echelons
% \node[rectangle, thick, draw=lightgray, minimum width = 103mm,text width=25mm, align=center,  minimum height = 0.9cm, anchor=west, dash pattern=on 0.2cm off 0.1cm] (r2) at (-1.5,-1.3) {\footnotesize\textit{Distribution}\vspace{18pt}};
% \node[rectangle, thick, draw=lightgray, minimum width = 103mm,text width=45mm, align=center, minimum height = 1.1cm, anchor=west, dash pattern=on 0.2cm off 0.1cm] (r1) at (-1.5,1.3) {\footnotesize\textit{Upstream sourcing}};
    
% \node[circle, thick, draw=lightgray, minimum width = 1.3cm, anchor=west, dash pattern = on 0.2cm off 0.1cm] (c1) at (-0.7,-1.8) {};
% \node[circle, thick, draw=lightgray, minimum width = 1.3cm, anchor=west, dash pattern = on 0.2cm off 0.1cm] (c2) at (2.3,-1.8) {};
% \node[circle, thick, draw=lightgray, minimum width = 1.3cm, anchor=west, dash pattern = on 0.2cm off 0.1cm] (c3) at (5.3,-1.8) {};

% \node[circle, thick, draw=lightgray, minimum width = 1.3cm, anchor=west, dash pattern = on 0.2cm off 0.1cm] (c4) at (-0.7, 1.8) {};
% \node[circle, thick, draw=lightgray, minimum width = 1.3cm, anchor=west, dash pattern = on 0.2cm off 0.1cm] (c5) at (2.3, 1.8) {};
% \node[circle, thick, draw=lightgray, minimum width = 1.3cm, anchor=west, dash pattern = on 0.2cm off 0.1cm] (c6) at (5.3, 1.8) {};
% \draw[thick, -, color=lightgray,dash pattern=on 0.2cm off 0.1cm] (r1) to (i1);
% \draw[thick, -, color=lightgray,dash pattern=on 0.2cm off 0.1cm] (r1) to (i2);
% \draw[thick, -, color=lightgray,dash pattern=on 0.2cm off 0.1cm] (c5) to (i1);
% \draw[thick, -, color=lightgray,dash pattern=on 0.2cm off 0.1cm] (c5) to (i2);



% \node [text width=3cm,right = 0.5cm of r1] (r1label) {\textit{Possible upstream echelons}};
% \node [text width=3.8cm,right = 0.5cm of r2] (r2label) {\textit{Possible intermediate echelons}};
% \draw (r2label.west) edge (r2.east) ;
% \draw (r2label.west) edge (r1.east) ;

\end{tikzpicture}

==> tikz/tikz_FastEstDirOpt.tex <==


\usetikzlibrary{shapes.geometric}
% Define block styles
\begin{tikzpicture}[
textnode1/.style={rectangle, draw=black!60, fill=white!0, thick, minimum height = 1.1cm,text width=2.5cm, align=left},
squarednode/.style={rectangle, draw=gray!60, fill=gray!25, very thick,minimum height = 1.5cm,text width=2.5cm, align=center},
squarednode2/.style={rectangle, draw=gray!60, fill=gray!25, very thick,minimum height = 1.5cm,text width=4.5cm, align=center},
squarednode3/.style={rectangle, draw=gray!60, fill=gray!25, very thick,minimum height = 1.5cm,text width=12cm, align=center},
rectnode/.style={rectangle, draw=blue!60, fill=blue!25, very thick,  minimum height = 1.5cm, text width=2.8cm, align=center},
rectnode2/.style={rectangle, draw=blue!60, fill=blue!25, very thick,  minimum height = 1.5cm, text width=2cm, align=center},
rectnode3/.style={rectangle, draw=blue!60, fill=blue!25, dashed,  minimum height = 5cm, text width=5cm, align=left},
rectnode4/.style={rectangle, draw=blue!60, fill=blue!25, dashed, thick,  minimum height = 3.85cm, text width=2.5cm, align=left},
rectnode5/.style={rectangle, draw=blue!60, fill=blue!25, dashed,  minimum height = 2.7cm, text width=1cm, align=left},
rectnode6/.style={rectangle, draw=blue!60, fill=blue!25, very thick,  minimum height = 6.15cm, text width=5.cm, align=left},
% node distance=10mm
]


%Nodes
\node[rectnode2](o3) {\footnotesize $\allocVec$, $\sourcingMat$};
\node[rectnode2](o2)[right = 1.0cm of o3] {\footnotesize $L(\cdot,\cdot)$};
\node[rectnode6](o6)[left = 2.4cm of o3]  {\footnotesize $\Gamma\overset{{\text{MCMC}}}{\sim}\dataSet$};
\node[rectnode4](o4)[left= 2.6cm of o3] { $\truthdraws$};
\node[rectnode5](o5)[left= 2.8cm of o3] { $\datadraws$};
\node[squarednode](p2)[below = 2.3cm of o3]  {\footnotesize Generate $\dataSetNext$};
\node[squarednode](p3)[below = 1.3cm of p2]  {\footnotesize Get binomial likelihood $\binomLikeMat_{ij}$};
\node[squarednode3](p4)[below = 6.5cm of o4]  {\footnotesize Return $\frac{1}{|\datadraws|}\sum_{j=1}^{|\datadraws|} \min_{\tnsnRatesEst} \bigg\{ \sum_{i=1}^{|\truthdraws|}\binomLikeMat_{ij}L(\tnsnRatesEst,\tnsnRates^{(i)}) \bigg\}$};
\node[textnode1](t1)[left= 5.2cm of p3]{\scriptsize SciPy optimizer, analytical solution };

%Lines
% \draw[thick,-] (i1) to  node[pos=0.5, left] {\normalsize{$\frac{3}{6}$}} (o1) ;
\draw[thick,->] (o5) -- + (2.8,-2.1) |-  node[pos=-0.05, above] {\normalsize{$\tnsnRates^{(j)}$}}  (p2) ;
\draw[thick,->] (o3) to  node {} (p2) ;
\draw[thick,->] (p2) to  node[pos=0.6, right] {$\dataSetNext$} (p3) ;
\draw[thick,->] (o4) -- + (2.5,-2.1) |-  node[pos=0.4, right] {\normalsize{$\tnsnRates^{(i)}$}}  (p3) ;
\draw[thick,->] (p3) to  node[pos=0.6, above] {$\binomLikeMat$} (p4) ;
\draw[thick,->] (o4) -- + (-0.3, -3.5) -|  node[pos=0.5, right] {\normalsize{$\tnsnRates^{(i)}$}}  (p4) ;
\draw[dashed,->] (t1) to  (-5.5,-9) ;
\draw[thick,->] (o2) -- + (-1.0,-2.1) |-  node {}  (p4) ;


%\draw[thick,->] (i1) to node[very near end,above] {{$\frac{0}{12}$}} (o2);
% \draw[thick,-] (p2) to node[pos=0.97, above] {} (o2);
% \draw[thick,-] (p2) to node[pos=0.85, right] {} (o3);
% \draw[thick,->] (i3) to node[right] {{$\frac{0}{12}$}} (o3);
% \draw[thick,->] (i3) to node[above] {{$\frac{0}{12}$}} (o2);

% Make a legend
% \matrix [draw,below left] at (current bounding box.south west) {
%   \node [roundnode,label=right:Foo] {}; \\
%   \node [squarednode,label=right:Bar] {}; \\
% };

% \node[draw,left = 1.5cm of o1,minimum height=1.1cm,minimum width=2.5cm] (lgd) {$\frac{\text{\footnotesize positive tests}}{\text{\footnotesize total samples}}$};

% Other possible echelons
% \node[rectangle, thick, draw=lightgray, minimum width = 103mm,text width=25mm, align=center,  minimum height = 0.9cm, anchor=west, dash pattern=on 0.2cm off 0.1cm] (r2) at (-1.5,-1.3) {\footnotesize\textit{Distribution}\vspace{18pt}};
% \node[rectangle, thick, draw=lightgray, minimum width = 103mm,text width=45mm, align=center, minimum height = 1.1cm, anchor=west, dash pattern=on 0.2cm off 0.1cm] (r1) at (-1.5,1.3) {\footnotesize\textit{Upstream sourcing}};
    
% \node[circle, thick, draw=lightgray, minimum width = 1.3cm, anchor=west, dash pattern = on 0.2cm off 0.1cm] (c1) at (-0.7,-1.8) {};
% \node[circle, thick, draw=lightgray, minimum width = 1.3cm, anchor=west, dash pattern = on 0.2cm off 0.1cm] (c2) at (2.3,-1.8) {};
% \node[circle, thick, draw=lightgray, minimum width = 1.3cm, anchor=west, dash pattern = on 0.2cm off 0.1cm] (c3) at (5.3,-1.8) {};

% \node[circle, thick, draw=lightgray, minimum width = 1.3cm, anchor=west, dash pattern = on 0.2cm off 0.1cm] (c4) at (-0.7, 1.8) {};
% \node[circle, thick, draw=lightgray, minimum width = 1.3cm, anchor=west, dash pattern = on 0.2cm off 0.1cm] (c5) at (2.3, 1.8) {};
% \node[circle, thick, draw=lightgray, minimum width = 1.3cm, anchor=west, dash pattern = on 0.2cm off 0.1cm] (c6) at (5.3, 1.8) {};
% \draw[thick, -, color=lightgray,dash pattern=on 0.2cm off 0.1cm] (r1) to (i1);
% \draw[thick, -, color=lightgray,dash pattern=on 0.2cm off 0.1cm] (r1) to (i2);
% \draw[thick, -, color=lightgray,dash pattern=on 0.2cm off 0.1cm] (c5) to (i1);
% \draw[thick, -, color=lightgray,dash pattern=on 0.2cm off 0.1cm] (c5) to (i2);



% \node [text width=3cm,right = 0.5cm of r1] (r1label) {\textit{Possible upstream echelons}};
% \node [text width=3.8cm,right = 0.5cm of r2] (r2label) {\textit{Possible intermediate echelons}};
% \draw (r2label.west) edge (r2.east) ;
% \draw (r2label.west) edge (r1.east) ;

\end{tikzpicture}
